Cooling Measures and Housing Wealth: Evidence from Singapore

Excessive house price growth was at the heart of the financial crisis in 2007/08. Since then, many countries have added cooling measures to their regulatory frameworks. It has been found that these measures can indeed control price growth, but no one has examined whether this has adverse consequences for the housing wealth distribution. We examine this for Singapore, which started in 2009 to target price growth over ten rounds in total. We find that welfare from housing wealth in the last round might not be higher than before 2009. This depends on the deflator used to convert nominal into real prices. Irrespective of the deflator, we can reject that welfare increased monotonically over the different rounds.

==> tables/table_equivalent_wealth.tex <==
\begin{table}[ph!]
\centering
\caption{{\bf Ratios of equivalent housing wealth for the different cooling rounds.} Ratio of estimated equivalent wealth for round $r$ to those estimated for base period 0. Significance levels based on bootstrapped p-values with $B=?$ replications. {\textcolor{red}{\bf RS: requires split for public and private sector.}}}
\label{tab:equivalent_wealth}
\begin{adjustbox}{max width = \textwidth}
\begin{tabular}{lrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{$\bsy{\nu}$} & \multicolumn{10}{c}{\bf Round }\\\cline{1-11}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\\cline{2-11}
 & \multicolumn{10}{c}{Deflator: CPI}\\\cline{2-11}
0.0 &&&&&&&&&&\\
1.0 &&&&&&&&&&\\
1.5 &&&&&&&&&&\\
2.0 &&&&&&&&&&\\
2.5 &&&&&&&&&&\\\cline{2-11}
 & \multicolumn{10}{c}{Deflator: Wage}\\\cline{2-11}
 0.0 &&&&&&&&&&\\
1.0 &&&&&&&&&&\\
1.5 &&&&&&&&&&\\
2.0 &&&&&&&&&&\\
2.5 &&&&&&&&&&\\\cline{2-11}
  & \multicolumn{10}{c}{Deflator: GNI}\\\cline{2-11}
 0.0 &&&&&&&&&&\\
1.0 &&&&&&&&&&\\
1.5 &&&&&&&&&&\\
2.0 &&&&&&&&&&\\
2.5 &&&&&&&&&&\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


